The Adjoint Petrov-Galerkin Method for Non-Linear Model Reduction

We formulate a new projection-based reduced-ordered modeling technique for non-linear dynamical systems. The proposed technique, which we refer to as the Adjoint Petrov-Galerkin (APG) method, is derived by decomposing the generalized coordinates of a dynamical system into a resolved coarse-scale set and an unresolved fine-scale set. A Markovian finite memory assumption within the Mori-Zwanzig formalism is then used to develop a reduced-order representation of the coarse-scales. This procedure leads to a closed reduced-order model that displays commonalities with the adjoint stabilization method used in finite elements. The formulation is shown to be equivalent to a Petrov-Galerkin method with a non-linear, time-varying test basis, thus sharing some similarities with the least-squares Petrov-Galerkin method. Theoretical analysis examining a priori error bounds and computational cost is presented. Numerical experiments on the compressible Navier-Stokes equations demonstrate that the proposed method can lead to improvements in numerical accuracy, robustness, and computational efficiency over the Galerkin method on problems of practical interest. Improvements in numerical accuracy and computational efficiency over the least-squares Petrov-Galerkin method are observed in most cases.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> proofs3.tex <==
\begin{theorem}
Let $\mathbf{R}(\ufullvec) = \mathbf{A}\ufullvec$ be a linear time-invariant operator. Error bounds for the coarse-scales in the Galerkin and APG ROMs, are, respectively,
\begin{equation}\label{eq:g_ltibound_inplane}
\norm{\errorcoarse_G(t) } \le  \norm{\mathbf{S}_G} \norm{\mathbf{S}_G^{-1} }\int_0^t  \norm{ e^{ \Lambda_{G} (t-s)}  } \norm{ \mathbb{P}_G \mathbf{r}_F (\ucoarsevec_F(s)) } ds ,
\end{equation}
\begin{equation}\label{eq:ag_ltibound_inplane}
\norm{\errorcoarse_A(t) } \le \norm{\mathbf{S}_A} \norm{\mathbf{S}_A^{-1} } \int_0^t \norm{ e^{ \Lambda_{A}(t-s)} } \norm{ \mathbb{P}_A \mathbf{r}_F (\ucoarsevec_F (s)) }ds ,
\end{equation}
where $\Lambda_{G}$ is a diagonal matrix of the eigenvalues of $\vcoarsevec^T \mathbb{P}_G \mathbf{A} \vcoarsevec$, while $\mathbf{S}_G$ are the eigenvectors of $\vcoarsevec^T \mathbb{P}_G \mathbf{A} \vcoarsevec$. Similar definitions hold for $\Lambda_{A}$ and $\mathbf{S}_A$ using the APG projection. 
\end{theorem}
\begin{proof}
We prove only Eq.~\ref{eq:ag_ltibound_inplane} as Eq.~\ref{eq:g_ltibound_inplane} is obtained through the same arguments. Subtracting Eq.~\ref{eq:ag_error} from Eq.~\ref{eq:fom_error}, and adding and subtracting $\mathbb{P}_A\mathbf{A} \ufullvec_F$,
%$$
%\frac{d \error_A}{dt} = \mathbf{A} \ufullvec_F + \mathbb{P}_A \mathbf{A} \ufullvec_F - \mathbb{P}_A %\mathbf{A} \ufullvec_F  - \mathbb{P}_A \mathbf{A}\ucoarsevec_G, \qquad \mathbf{e}_A(0) = \mathbf{0}.
%$$
%Gathering terms,
$$
\frac{d \error_A}{dt} = \big[\mathbf{I} - \mathbb{P}_A \big]  \mathbf{A} \ufullvec_F  +  \mathbb{P}_A \mathbf{A} \error_A, \qquad \mathbf{e}_A(0) = \mathbf{0}.
$$
Decomposing the error into coarse and fine-scale components,
$$\error_A = \errorcoarse_A + \errorfine_A.$$
Since $\ufinevec_A = 0$ for all time, $\errorfine_A = \ufinevec_{F}$.
An equation for the coarse-scale error is obtained by left multiplying by $\vcoarsevec^T \mathbb{P}_A$,
$$
\vcoarsevec^T \mathbb{P}_A \frac{d \errorcoarse_A}{dt} + \vcoarsevec^T \mathbb{P}_A \frac{d \errorfine_A}{dt} = \vcoarsevec^T \mathbb{P}_A \big[\mathbf{I} - \mathbb{P}_A \big]  \mathbf{A} \ufullvec_F  +  \vcoarsevec^T \mathbb{P}_A  \mathbb{P}_A \mathbf{A} \errorcoarse_A + \vcoarsevec^T \mathbb{P}_A \mathbb{P}_A \mathbf{A} \ufinevec_{F}.
$$
Define the generalized coordinates for the coarse-scale error as,
$$\errorcoarsegen_A  = \vcoarsevec^T \errorcoarse_A, \qquad \errorcoarsegen_A \in \mathbb{R}^K.$$
Rearranging gives,
$$
\frac{d \errorcoarsegen_A}{dt}  = \vcoarsevec^T \mathbb{P}_A \big[\mathbf{I} - \mathbb{P}_A \big]  \mathbf{A} \ufullvec_F  +  \vcoarsevec^T \mathbb{P}_A  \mathbb{P}_A \mathbf{A} \errorcoarse_A + \vcoarsevec^T \mathbb{P}_A \mathbb{P}_A \bigg( \mathbf{A} \ufinevec_{F} - \frac{d \ufinevec_F}{dt} \bigg).
$$
Noting that $\mathbb{P}_A^2 = \mathbb{P}_A$, the first term on the right-hand side is zero, and the equation reduces to,
\begin{equation}\label{eq:lti_inplane}
\frac{d \errorcoarsegen_A}{dt} = \vcoarsevec^T \mathbb{P}_A \mathbf{A} \vcoarsevec \errorcoarsegen_A + \vcoarsevec^T \mathbb{P}_A \bigg(  \mathbf{A} \ufinevec_{F} -  \frac{d \ufinevec_F}{dt}\bigg).
\end{equation}
Equation~\ref{eq:lti_inplane} is a first-order linear inhomogeneous differential equation that can be solved analytically. A standard way to do this is by performing the eigendecomposition,
%Performing triangle inequality and noting the first term is zero,
%\begin{equation}\label{eq:eg_lti}
%\frac{d \norm{ \errorcoarsegen_A }}{dt} \le \norm{ \vcoarsevec^T \mathbb{P}_A \mathbf{A} \vcoarsevec \errorcoarsegen_A }+ \norm{\vcoarsevec^T \mathbb{P}_A \mathbf{A} \ufinevec_{F}}.
%\end{equation}
%By the submultipicative property of the 2-norm,
%\begin{equation}\label{eq:eg_lti}
%\frac{d \norm{ \errorcoarsegen_A }}{dt} \le \norm{ \vcoarsevec^T \mathbb{P}_A \mathbf{A} \vcoarsevec} \norm{ \errorcoarsegen_A }+ \norm{\vcoarsevec^T \mathbb{P}_A \mathbf{A} \ufinevec_{F}}.
%\end{equation}
%Noting that $\norm{ \errorcoarsegen_A} = \norm{\vcoarsevec^T \error_A} = \norm{\error_A}$,
%\begin{equation}\label{eq:eg_lti_bound}
%\frac{d \norm{\errorcoarse_A} }{dt} \le \norm{ \vcoarsevec^T \mathbb{P}_A \mathbf{A} \vcoarsevec} \norm{ \errorcoarse_A }+ \norm{\vcoarsevec^T \mathbb{P}_A \mathbf{A} \ufinevec_{F}}.
%\end{equation}
%Equation~\ref{eq:eg_lti_bound} is a linear homogeneous first order equation and has the solution,
%\begin{equation}\label{eq:eg_lti}
%\errorcoarse(t) \le \int_0^t e^{ \norm{ \vcoarsevec^T \mathbb{P}_A \mathbf{A} \vcoarsevec}s}\norm{\vcoarsevec^T \mathbb{P}_A \mathbf{A} } \norm{\ufinevec_{F}(t-s) ds } .
%\end{equation}
$$\vcoarsevec^T \mathbb{P}_A \mathbf{A} \vcoarsevec = \mathbf{S_A}\Lambda_A \mathbf{ S_A^{-1} },$$
where $\mathbf{S}_A \in \mathbb{R}^{K \times K}$ are the eigenvectors and $\Lambda_A$ is a diagonal matrix of eigenvalues.
Equation~\ref{eq:lti_inplane} can be written as,
 \begin{equation}\label{eq:eg_lti_1}
\frac{d \errorcoarsegen_A}{dt} =\mathbf{S_A}\Lambda_A \mathbf{ S_A^{-1} } \errorcoarsegen_A + \vcoarsevec^T \mathbb{P}_A \bigg(  \mathbf{A} \ufinevec_{F} -  \frac{d \ufinevec_F}{dt}\bigg),
\end{equation}
Left multiplying by $\mathbf{S_A}^{-1}$ to obtain a set of decoupled equations,
 \begin{equation}\label{eq:eg_lti_2}
\frac{d \mathbf{w}_A}{dt} =  \Lambda_A \mathbf{w}_A + \mathbf{S_A}^{-1} \vcoarsevec^T \mathbb{P}_A \bigg(  \mathbf{A} \ufinevec_{F} -  \frac{d \ufinevec_F}{dt}\bigg),
\end{equation}
where $\mathbf{w}_A = \mathbf{S}^{-1} \errorcoarsegen_A$. 
The above is a set of decoupled first order inhomogenous differential equation that have the solution,
$$
\mathbf{w}_A(t) = \int_0^t e^{ \Lambda_A s}  \mathbf{S_A}^{-1} \vcoarsevec^T \mathbb{P}_A \bigg(  \mathbf{A} \ufinevec_{F}(t-s) -  \frac{d }{dt}\ufinevec_F(t-s)\bigg) ds. 
$$
Left multiplying by $\vcoarsevec \mathbf{S_A}$ to obtain an equation for the coarse-scale error,
$$
\errorcoarse_A = \int_0^t \vcoarsevec  \mathbf{S_A} e^{ \Lambda_A (t-s)}  \mathbf{S_A}^{-1} \vcoarsevec^T \mathbb{P}_A \bigg(  \mathbf{A} \ufinevec_{F}(s) -  \frac{d }{dt}\ufinevec_F(s)\bigg) ds.
$$
By definition of the FOM,
$$\frac{d \ucoarsevec_F}{dt} + \frac{d \ufinevec_F}{dt} = \mathbf{A}\ucoarsevec_F + \mathbf{A}\ufinevec_F.
$$
Thus,
$$
\errorcoarse_A = \int_0^t \vcoarsevec  \mathbf{S_A} e^{ \Lambda_A (t-s)}  \mathbf{S_A}^{-1} \vcoarsevec^T \mathbb{P}_A \bigg(\frac{d }{dt}\ucoarsevec_F(s) - \mathbf{A} \ucoarsevec_F(s) \bigg) ds.
$$
Using the definition of the residual,
$$
\errorcoarse_A = \int_0^t \vcoarsevec  \mathbf{S_A} e^{ \Lambda_A (t-s)}  \mathbf{S_A}^{-1} \vcoarsevec^T \mathbb{P}_A \mathbf{r}(\ucoarsevec(s) )ds.
$$
Taking the norm and using the sub-multiplicative property,
$$
\norm{ \errorcoarse_A } \le \int_0^t \norm{ \vcoarsevec  \mathbf{S_A} e^{ \Lambda_A (t-s)}  \mathbf{S_A}^{-1} } \norm{ \vcoarsevec^T \mathbb{P}_A \mathbf{r}(\ucoarsevec(s) ) }ds.
$$

\end{proof}
Similar to the non-linear case, Eqns~\ref{eq:g_ltibound_inplane} and~\ref{eq:g_ltibound_inplane} contain two distinct terms. The first term corresponds to the exponential growth in time, $e^{\Lambda_A s}$. In contrast to the non-linear case, however, the arguments in the exponential contain the eigenvalues of $\vcoarsevec^T \mathbb{P}_A \mathbf{A} \vcoarsevec$. When these eigenvalues are negative, the term $e^{\Lambda_A s}$  can diminish the growth of error in time. The second term of interest is given by $\norm{ \mathbb{P}_A \mathbf{A} } \norm{ \ufinevec_{F}(t) }$. This term corresponds to the error introduced due to the unresolved scales at time $t$. This term is a statement of the error introduced due to the closure problem. 

\begin{corollary}\label{corollary:lti_corollary}
Let $\mathbf{R}(\ufullvec) = \mathbf{A}\ufullvec$ be a linear time-invariant operator. If $\norm{\mathbb{P}_A \mathbf{r}(\ucoarsevec(t) ) } \le \norm{\mathbb{P}_G \mathbf{r}(\ucoarsevec(t) ) }$, then the upper bound on how much error is introduced due to the fine-scales is less for APG than for the Galerkin Method.
\end{corollary}
\begin{proof}

\end{proof}
Corollary~\ref{corollary:lti_corollary} shows that it is possible for the APG method to be more accurate than the Galerkin method. %In general, $\norm{ \mathbf{A} + \tau \mathbf{A} \Pifine \mathbf{A} }$ will depend on the structure of $\mathbf{A}$ (symmetry, eigenvalues, etc.)  Theorem~\ref{theorem:errorbound_symmetric} examines one possible situation in which Corollary~\ref{corollary:lti_corollary} is relevant.
\begin{theorem}\label{theorem:errorbound_symmetric}
Let $\mathbf{R}(\ufullvec) = \mathbf{A}\ufullvec$ be a linear time-invariant operator. If $\mathbf{A}$ is self-adjoint with all real negative eigenvalues, then $\kappa_1 \le 0$ and  $\norm{\mathbf{A} + \tau \mathbf{A} \Pifine \mathbf{A}  } \le \norm{ \mathbf{A} }$ for $\tau \le \frac{\lambda_1}{\lambda_N^2}$, where $\lambda_1$ and $\lambda_N$ are the largest and smallest eigenvalues of $\mathbf{A}$, respectively, and $\kappa_1$ is the largest eigenvalue of $\mathbf{A} + \tau \mathbf{A} \Pifine \mathbf{A}.$
\end{theorem}

\begin{proof}
%Note that,
%$$\norm{ \vcoarsevec^T \mathbb{P}_A \mathbf{A} \vcoarsevec } \le \norm{\vcoarsevec^T} \norm{\mathbb{P}_A \mathbf{A}}  \norm{\vcoarsevec^T} = \norm{\mathbb{P}_A \mathbf{A} } ,$$
%and the same for $\norm{\mathbb{P}_G \mathbf{A}}$. It is thus sufficient to prove,
%$$ \norm{ \vcoarsevec^T \mathbb{P}_A \mathbf{A} \vcoarsevec } \le \norm{ \vcoarsevec^T \mathbb{P}_G \mathbf{A} \vcoarsevec }.$$ 
Start by determining $\norm{\mathbf{A}}$. 
As $\mathbf{A}$ is symmetric, the $2$-norm is equivalent to the spectral radius,
$$\norm{ \mathbf{A}} = \rho( \mathbf{A} ).$$
Let $\lambda_1 \ge \lambda_2 \ge \hdots \ge \lambda_N$ be the $N$ eigenvalues of $ \mathbf{A} $. As all eigenvalues are negative, it directly follows that,
$$\norm{ \mathbf{A} } = |\lambda_N|.$$

Having obtained an expression for $\norm{ \mathbf{A} }$, the goal now is to obtain an upper bound on $\norm{ \mathbf{A} + \tau \mathbf{A} \Pifine \mathbf{A} }$. It is seen that, if $\mathbf{A}$ is self-adjoint, so is $ \mathbf{A} + \tau \mathbf{A} \Pifine \mathbf{A} $. As such, 
$$\norm{\mathbf{A} + \tau \mathbf{A} \Pifine \mathbf{A}  } = \rho( \mathbf{A} + \tau \mathbf{A} \Pifine \mathbf{A} ).$$
Let $\kappa_1 \ge \kappa_2 \ge \hdots \kappa_N$ be the $N$ eigenvalues of $\mathbf{A} + \tau \mathbf{A} \Pifine \mathbf{A}$ Then,
$$\rho(\mathbf{A} + \tau \mathbf{A} \Pifine \mathbf{A} ) = \text{max}(|\kappa_1|,|\kappa_N|).$$
Thus the objective is to find a lower bound on $\kappa_N$, an upper bound on $\kappa_1$, and find $\tau$ such that these bounds are lower than $|\lambda_N|$ and 0, respectively. Let $\gamma_1 \ge \gamma_2 \ge \hdots \ge \gamma_N$ be the $N$ eigenvalues of  $\mathbf{A} \Pifine \mathbf{A}$. %  and $\lambda_i$ be the $i_{th}$ largest eigenvalue of $\mathbf{A}.$   
%As both $\mathbf{A}$ and $\mathbf{A} \Pifine \mathbf{A}$ are self-a djoint, the Weyl inequalities can be used to bound the smallest and largest eigenvalue of $\mathbb{P}_A \mathbf{A}$,
As all matrices are self-adjoint, the Weyl inequalities can be used to bound the smallest and largest eigenvalue of $\mathbf{A} + \tau \mathbf{A} \Pifine \mathbf{A}$,
\begin{equation}\label{eq:weyl_large}
\kappa_1 \le \lambda_1 + \tau \gamma_1,
\end{equation}
\begin{equation}\label{eq:weyl_small}
\kappa_N \ge \lambda_N + \tau \gamma_N.
\end{equation}
As $\mathbf{A} \Pifine \mathbf{A}$ is positive semi-definite, $\gamma_i > 0 \text{ for } i = 1,2,\hdots,N$, it then directly follows from Eq.~\ref{eq:weyl_small} that, 
$$\kappa_N \ge \lambda_N \qquad \forall \tau \ge 0.$$
Thus, for all $\tau \ge 0$ the smallest eigenvalue of $\mathbf{A} + \tau \mathbf{A} \Pifine \mathbf{A} $ is larger than or equal to the smallest eigenvalue of $ \mathbf{A}$ and,
$$|\kappa_N| \le |\lambda_N| ; \qquad \forall \tau \ge 0.$$
For the largest eigenvalue, it follows from Eq.~\ref{eq:weyl_large} that to obtain the desired result one requires,
$$\kappa_1 \le \lambda_1 + \tau \gamma_1  \le 0,$$
which gives the following relation,
\begin{equation}\label{eq:ineq_1}
\kappa_1 \le 0; \qquad \forall \tau \le \frac{-\lambda_1}{\gamma_1}.
\end{equation}
As $\gamma_1 \ge 0$ and $\lambda_1 \le 0$, the conditions required for $\norm{\mathbf{A} + \tau \mathbf{A} \Pifine \mathbf{A} } \le \norm{ \mathbf{A} }$ and $\kappa_1 \le 0$ provided sufficiently small $\tau$ have been met. To write the bounds on $\tau$ in Eq.~\ref{eq:ineq_1} into a more intiutive form, the eigenvalue, $\gamma_1$, can be related to $\lambda_i$ through the the Weyl inequalities. Noting that $\gamma_i$ are the eigenvalues of,
$$\mathbf{A} \Pifine \mathbf{A}  =  \mathbf{A}^2 - \mathbf{A} \Picoarse \mathbf{A}.$$
As $\mathbf{A} \Picoarse \mathbf{A}$ is positive semi-definite, one has,
\begin{equation}\label{eq:weyl3}
\gamma_1 \le \lambda_N^2.
\end{equation}
Inserting the above inequality into Eq.~\ref{eq:ineq_1}, one obtains the desired result,
\begin{equation}\label{eq:tau_bound}
\kappa_1 \le 0; \qquad \forall \tau \le \frac{| \lambda_1 | }{\lambda_N^2}.
\end{equation}
%Lastly, noting that $\mu_1 \le \lambda_1$ (again by the Poincar\'e separation theorem), one obtains the final result.
%\begin{equation}\label{eq:tau_bound}
%\norm{\mathbb{P}_A \mathbf{A} } \le \norm{ \mathbb{P}_G \mathbf{A} };  \qquad \forall \tau \le \frac{| \lambda_1 | }{\lambda_N^2}.
%\end{equation}
\end{proof}

\begin{corollary}\label{corollary:eigs}
Let $\mathbf{R}(\ufullvec) = \mathbf{A}\ufullvec$ be a linear time-invariant operator. If $\mathbf{A}$ is self-adjoint with all real negative eigenvalues, then $\eta_i \ge \mu_i$ for $i = 1,2,\hdots,K$, where $\eta_1 \ge \eta_2 \hdots \ge \eta_K$ are the $K$ eigenvalues of $\vcoarsevec^T \mathbb{P}_A \mathbf{A} \vcoarsevec$ and $\mu_1 \ge \mu_2 \hdots \ge \mu_K$ are the $K$ eigenvalues of $\vcoarsevec^T \mathbb{P}_G \mathbf{A} \vcoarsevec$.
\end{corollary}

\begin{proof}
The proof follows the steps exactly given in Theorem~\ref{theorem:errorbound_symmetric}, but seeks bounds on the matrices $\vcoarsevec^T \mathbb{P}_G\mathbf{A} \vcoarsevec$ and $\vcoarsevec^T \mathbb{P}_A \mathbf{A} \vcoarsevec$ (opposed to $\mathbf{A}$ and $\mathbf{A} + \tau \mathbf{A} \Pifine \mathbf{A}$).
\end{proof} 

Theorem~\ref{theorem:errorbound_symmetric} and Corollary~\ref{corollary:eigs} contain three interesting results that will be  discussed. First, as discussed in Corollary~\ref{corollary:lti_corollary}, Theorem~\ref{theorem:errorbound_symmetric} shows that, for a sufficiently small value of $\tau$, the upper-bound on the error introduced at time $t$ due to the fine-scales is less in APG than in Galerkin. This is an appealing result as APG is derived as a subgrid-scale model. The next interesting result of Theorem~\ref{theorem:errorbound_symmetric} and Corollary~\ref{corollary:eigs} is that the maximum (least negative) eigenvalue in the exponential term in Eqns~\ref{eq:g_ltibound_inplane} and~\ref{eq:ag_ltibound_inplane} is larger for APG than Galerkin. This implies that APG is less dissipative than Galerkin, and means that errors may be slower to decay in time. Finally, Theorem~\ref{theorem:errorbound_symmetric} shows that the bounds on the parameter $\tau$ depends on the spectral content of the Jacobian of $\mathbf{A}$. This observation has been made heuristically in Ref~\cite{parishMZ1}. While Eq.~\ref{eq:tau_bound} provides insight into the selection and behaviour of $\tau$, it provides a conservative upper-bound on $\tau$ due to the repeated use of inequalities.




